Multi-resource Energy-efficient Routing in Cloud Data Centers with Networks-as-a-Service

With the rapid development of software defined networking and network function virtualization, researchers have proposed a new cloud networking model called Network-as-a-Service (NaaS) which enables both in-network packet processing and application-specific network control. In this paper, we revisit the problem of achieving network energy efficiency in data centers and identify some new optimization challenges under the NaaS model. Particularly, we extend the energy-efficient routing optimization from single-resource to multi-resource settings. We characterize the problem through a detailed model and provide a formal problem definition. Due to the high complexity of direct solutions, we propose a greedy routing scheme to approximate the optimum, where flows are selected progressively to exhaust residual capacities of active nodes, and routing paths are assigned based on the distributions of both node residual capacities and flow demands. By leveraging the structural regularity of data center networks, we also provide a fast topology-aware heuristic method based on hierarchically solving a series of vector bin packing instances. Our simulations show that the proposed routing scheme can achieve significant gain on energy savings and the topology-aware heuristic can produce comparably good results while reducing the computation time to a large extent.

==> design.tex <==
%!TEX root = main.tex
\section{GreenNaaS}
\label{sec:design}

In this section, we first provide the an overview for the general design of GreenNaaS and then, we detail its main components.

\subsection{Design Overview}

The architecture of GreenNaaS is simply constructed taking advantage of the central controlling manner of SDN. An overview can be found in Fig.~\ref{fig:green-naas}. GreenNaaS consists of three main components: the monitor, the optimizer, and the controller.

\begin{figure}[!h]
\centering
\includegraphics[scale=0.35]{./fig/green-naas.pdf}
\caption{\label{fig:green-naas}An overview of GreenNaaS.}
\end{figure}

The monitor keeps sensing the changes on the set of flows on the network over time. When there is a noticeable change happens, the topology information, together with the new set of detected flows will be pushed to the optimizer. After solving a minimum-energy optimization problem, the optimizer outputs to the controller the set of nodes that should sustain active, as well as the routing decisions for the flows. The controller then notifies the unnecessary nodes to sleep while keeping the controller-node communication channel active and installs routing entries in the active nodes with a processing function specified for every flow. Although GreenNaaS has distinct functionalities in its main components compared to existing architectures such as ElasticTree, they share similar processing logics. Due to this fact, we don't claim any contribution on the novelty of the architecture itself.

\subsection{Main Components}

{\bf The monitor.}~~The monitor is in charge of sensing the dynamic of the set of flows on the network. This can be accomplished by running a monitoring process at the edge. When a new flow arrives at an edge node, the monitoring process at this node will generate a request to the monitor with the whole information of this flow, and this flow will be appended to a list of all active flows on the network. The monitor also maintains the topology information of the network, which can be directly inherited from the SDN controller.


{\bf The optimizer.}~~When receiving the list of flows and the topology information, the optimizer is dedicated to calculate the optimal set of active nodes and the routes for all the flows by solving an multi-resource energy-aware routing problem. After solving the optimization problem, the optimizer will output the candidate set of active nodes, as well as the routing decision made for each flow. All of these will be sent to the controller. We will formally define the optimization problem and elaborate our solution in detail in the next two sections. 

{\bf The controller.}~~The controller is responsible for two tasks: installing flow entries (with processing function specified for each flow) in nodes and changing the states of nodes. To this end, traditional control plane-data plane API such as OpenFlow has to be extended in order to support more application-specific manipulations on nodes.




==> naas.tex <==
%!TEX root = main.tex
\section{Background on Network-as-a-Service}
\label{sec:naas}

In this section, we provide the background information about the NaaS concept by summarizing the current states of SDN and software packet processing. Then, we describe the detail of NaaS and reveal some new research challenges.

{\bf Software defined networking.}
Traditional computer networks are conducted on proprietary network devices (from routers and switches to middleboxes) with complex, distributed control software running inside. The high-level coupling of the control plane (which decides how to handle the traffic) and the data plane (which forwards traffic according to decisions from the control plane) brings very high complexity to network management and leads to a very slow pace of development and evolution of network functionalities due to the reliance on specialist hardware.

SDN is obligated to solve these problems by changing the design and management of a network in the following two ways: in an SDN, the control plane and the data plane are clearly separated; the control plane is logically consolidated. The control plane thus exercises a full view of the network and can be implemented with a single software control program. Through a well-defined API such as OpenFlow, the control plane carries out direct control to push decisions over multiple data-plane elements in the network. The logically centralized controlling can facilitate most of the network applications including network virtualization \cite{Sherwood-Gibb}, dynamic access control \cite{Casado-Freedman, Nayak-Reimers}, server load balancing \cite{Wang-Butnariu}, and energy-efficient networking \cite{Heller-Seetharaman, Wang-Zhang-jsac} which would require enormous efforts to be implemented in a totally distributed environment.


{\bf Software packet processing.}
While SDN has helped speed up innovation in network control plane, fast innovation in data plane also becomes important due to the diverse networking requirements from cloud applications. Recently, researchers have argued for building evolvable networks, whose functionality changes with the needs of its users and is not tied to particular hardware vendors. An inexpensive way of building such networks is to run a network-programming framework such as Click on top of commodity general-purpose hardware, which is called general-purpose networking. There have been several research prototypes demonstrating that general-purpose hardware is capable of high-performance packet processing when the workloads are assume to be uniform and packets are subjected to single particular type of processing, such as IP forwarding \cite{Fall_Iannaccone-2011}, GPU-based IP forwarding \cite{Han_Jang-2010}, packet classification \cite{Ma_Banerjee-2010}, or cryptographic operations \cite{Jang_Han-2011}. It has also been shown in \cite{Dobrescu_Argyraki-2012} that such a software packet processing platform can achieve predictable performance while running various packet-processing applications and serving multiple clients with different needs.

{\bf NaaS architecture.}
An overview of the NaaS architecture is depicted in Fig.~\ref{fig:naas}. The network is conducted on an SDN implementation where a centralized controller takes charge of flow management including assigning routing paths and interposing network functions. The network is comprised of general-purpose servers with multiple network ports connected by high-speed links. In each node in the network, network functions for packet processing are virtualized and can be invoked by the controller by upper-layer applications according to their needs. The whole picture is similar to SODA \cite{Li_Yu-2014}, which is a network architecture recently proposed to enhance the data plane functionality of SDN. Based on the NaaS architecture, there are some new challenges that need further research efforts, most of which are optimization problems such as multi-resource traffic engineering for load balancing and network functions organization. In this paper, we focus on the multi-resource routing for energy minimization.

\begin{figure}[!t]
\centering
\includegraphics[scale=0.32]{./fig/naas.pdf}
\caption{\label{fig:naas}The fundamental architecture for NaaS in a typical cloud data center. Network control plane is separated from data plane by SDN while data plane can be customized through NFV.}
\end{figure}












